Classifying Network Vendors at Internet Scale

In this paper, we develop a method to create a large, labeled dataset of visible network device vendors across the Internet by mapping network-visible IP addresses to device vendors. We use Internet-wide scanning, banner grabs of network-visible devices across the IPv4 address space, and clustering techniques to assign labels to more than 160,000 devices. We subsequently probe these devices and use features extracted from the responses to train a classifier that can accurately classify device vendors. Finally, we demonstrate how this method can be used to understand broader trends across the Internet by predicting device vendors in traceroutes from CAIDA's Archipelago measurement system and subsequently examining vendor distributions across these traceroutes.

==> sections/ml.tex <==
\section{\mbox{Classifying Network Devices}}
\label{sec:ml}

To classify network devices at scale, we need to compile a set of probes that elicit unique
responses from each network device vendor, extract a set of features from the
responses, and train a model to distinguish the vendors
using those features. There are many challenges to fingerprinting network devices at
scale which must be acknowledged. A subset of devices are not visible at the
IP layer, and some devices may not respond to probe-based measurements. We
cannot fingerprint these devices with our techniques.
Furthermore, a single IP-visible device can be associated with multiple IP
addresses. We mitigate double counting labeled devices by dealiasing IP addresses
to a single device. Finally, we must use our smaller set of labeled devices,
which may not fully represent the larger set of unlabeled devices, to train a
model for classifying unlabeled devices. We acknowledge there may be bias in
our labeled dataset but still believe it to be the most principled approach to
tackle the challenge of classifying network devices at scale.

\subsection{Network Device Probes and Features}

Many devices, such as web servers, have a standard port that is open for
connections. Many network devices, on the other hand, have no such port. One option is to
find an open port by scanning the ports of each device before probing.
Unfortunately, this is not scalable and, even worse, many network devices may \emph{have
no open ports at all}. As such, we only consider probes that
either require no port or that are specifically sent to closed ports
on the target machine.

\subsubsection{Nmap}

\textbf{Probes.} Nmap is perhaps the most popular active OS fingerprinting tool and has been
developed for over 20 years~\cite{nmap}. Nmap's OS fingerprinting system is
thorough, first scanning the 1,000 most popular open ports on a device to find an
open port. It then sends up to 16 specially crafted TCP, UDP, and ICMP probes to
the device that are intended to invoke a unique response. While 10 of these
probes are sent to an open port, 6 of these probes (3 TCP, 1 UDP, 2
ICMP) are sent specifically to a closed port on the device. The 3 TCP probes
differ in their options and flags, the UDP probe is sent to elicit an ICMP error
message from the remote device, and the 2 ICMP packets are ICMP echo packets
with differing types and IP header values. More details on these probes can be
found in \Fref{app:nmap}. We use these 6 probes as a base set of
probes to send to each IP address.

\textbf{Probe implementation.} We directly port the Nmap closed port probes
above into Zmap to facilitate fingerprinting large amounts of devices
quickly~\cite{durumeric2013zmap}.

\textbf{Feature extraction.} Nmap transforms the responses it receives into
features by applying a series of tests on each
packet. These tests have been developed for over 20 years.
\Fref{tab:features} in \Fref{app:class} shows the list of features
that correspond to the closed port probes that we use for the scans. These features include the options and order of options in
the TCP headers, the behavior of the sequence and acknowledgment numbers in the
TCP responses, and the IP initial time-to-live of the responses.

\subsubsection{ICMP}

\textbf{Probes.} ICMP provides a unique avenue for useful probes as the protocol is not directed
to a particular port, meaning we can send an ICMP message to a network device with no
open ports and still receive a response. Furthermore, some network device OSes may restrict
access to valid ICMP requests that can be used for fingeprinting, such as ICMP
timestamp requests, giving insight into the
vendor of the device just by the response (or lack thereof) to the
probe~\cite{kohno2005remote}. While Nmap incorporates ICMP probes in
its fingerprinting system, it only sends two ICMP echo probes, omitting a wide variety of ICMP messages that can be
sent.

We expand on the set of probes that we can use for fingerprinting
through ICMP fuzzing. More specifically, the ICMP protocol contains a
\emph{type} field that currently has 34 standardized types. Many of these types contain
a \emph{code} field that specifies sub-types of each message, such as an
explanation for the error that was returned. We enumerate these standardized
types and codes by sending a valid ICMP message for each pair to each device
in the labeled
dataset.

\textbf{Probe implementation.} We develop an ICMP fuzzing system using
Scapy that sends a valid ICMP message for each implemented ICMP
type and code to each remote device~\cite{scapy}.

\textbf{Feature extraction.} We extract each header field and value of the ICMP
responses and encode them as a categorical feature for the fingerprints. A
subset of these features are shown in \Fref{tab:features} in \Fref{app:class}.
Features include the type and code of the ICMP response, the data in the address mask
reply, as well as the ICMP ID and sequence number fields.

\subsection{Network Device Classification}

We use the dataset of labeled network devices (\Fref{tab:gt}), and our set
of probes and features to train a model that predicts the class of a
fingerprint. In this section, we outline our choice of model, methods use to train the
model, and metrics for evaluating the trained model.

\subsubsection{Model}

We consider each feature extracted in \Fref{tab:features} as a categorical
feature. We use a one-hot-encoding (OHE) to transform each categorical feature
into \textit{n} binary features, where \textit{n} is the number of unique values
found in the original categorical feature. We use a random forest model for
classification, motivated by the expectation that specific feature interactions will be
important for performance. Furthermore, choosing a random forest model allows us to easily
interpret which features are driving the performance of the trained model.

\subsubsection{Metrics}

We evaluate the trained models using accuracy, ROC AUC, and F1 scores.
More specifically, we use a \textit{balanced accuracy score} to account for any class imbalance in the data, in which each sample is weighted according to the inverse prevalence of its true class.
This dataset represents a  multiclass classification problem.
We consider ROC scores in a ``one-vs-rest'' fashion, where each class \textit{C} is considered as a binary classification task between \textit{C} and all other classes.
Furthermore, we use a ``micro'' averaged F1 score, which counts the total number of true positives, false positive, and false negatives. We present the average metrics for a five-fold cross validation.

\subsubsection{Pipeline Evaluation}

We probe each IP address in the labeled dataset,
retrying each probe up to three times. For each probe requiring a port, we
choose a high numbered port at random for each scan (every IP is scanned on the
same ports). Choosing a high-numbered port increases the likelihood of the port
being closed. At this
point, we remove any IP address from the labeled dataset that did not respond to
any probes. After removing unresponsive IP addresses, we dealias the network devices
using the topology provided by CAIDA's ITDK. We then filter the number of
vendors down to the final set shown in \Fref{tab:gt} by examining a large
reduction in vendor labels ($\sim$500 devices) from the 11th most labeled vendor
vendor to the 12th. We do not consider devices outside of these 11 classes for our
evaluation.

To address the class imbalance (\Fref{tab:gt}), we balance the classes before training the model to avoid
trivializing the task for the model (learning to predict everything as Cisco).
Specifically, we downsample the Cisco and Mikrotik classes to 17,000 samples, which is in line with the 3rd most prevalent class in the dataset.

We use scikit-learn's implementation of a random forest classifier to train and test models~\cite{pedregosa2011scikit}.
One-hot encoding each feature in \Fref{tab:features} results in more than 1,000 features.
Scikit-learn's random forest implementation computes the importance of each feature in the model using the Gini feature importance, which we use to better understand the model.
We perform a randomized hyperparameter search of 50 different models, varying the number and depth of trees, the maximum number of features used by the trees, the minimum samples reqiured for internal and leaf nodes, if bootstrapping is used, and the function used to measure split quality.
We perform three-fold cross validation on each model where each fold preserves the percentage of the samples in each class across the entire dataset.
We choose the best performing model with respect to test accuracy to evaluate using five-fold cross validation.

\input{figures/tables/ml.tex}

\Fref{tab:ml-results} shows the mean accuracy, ROC AUC, and F1 scores resulting from five-fold cross validation using different sets of features.
Here, we note that the dataset contains 11 classes, so a random guess of the class by the model would results in approximately 9\% balanced accuracy score.
\Fref{tab:ml-results} shows that Nmap's closed port probes perform well on their own, reaching an F1 score of over 85\%.
Furthermore, we see ICMP fuzzing was relatively successful, but not as accurate as the more nuanced Nmap probes.
We inspect the features of the ICMP model to determine which probes are driving its performance.
Ultimately, three probes contribute to almost all of the model's performance: the ICMP echo probe, the ICMP timestamp probe, and the ICMP address mask probe.
We train the final model using Nmap's closed port features, the ICMP address mask probe, and the ICMP timestamp probe (Nmap's probes already contain two ICMP echo probes).
We see that adding these two probes improves the accuracy of the classifier by over 13\%, and the F1 score of the classifier by 6\% to 93\%.
Overall, by only sending 8 network packets to a closed port, with our methodology, we can identify a device vendor with 91.9\% balanced accuracy.
\Fref{fig:rocpr} in \Fref{app:class} shows ROC and PR curves of the final model.

Finally, we examine the model to determine which features are important.
\Fref{tab:features} shows the feature ranking of each feature in the classifier.
We see that the most important feature for the classifier is the initial TTL of the packet sent in response to the probes.
We also see that many of the features added from ICMP fuzzing lie in the top 10 features of the classifier.

